DeepLiDARFlow: A Deep Learning Architecture For Scene Flow Estimation Using Monocular Camera and Sparse LiDAR

Scene flow is the dense 3D reconstruction of motion and geometry of a scene. Most state-of-the-art methods use a pair of stereo images as input for full scene reconstruction. These methods depend a lot on the quality of the RGB images and perform poorly in regions with reflective objects, shadows, ill-conditioned light environment and so on. LiDAR measurements are much less sensitive to the aforementioned conditions but LiDAR features are in general unsuitable for matching tasks due to their sparse nature. Hence, using both LiDAR and RGB can potentially overcome the individual disadvantages of each sensor by mutual improvement and yield robust features which can improve the matching process. In this paper, we present DeepLiDARFlow, a novel deep learning architecture which fuses high level RGB and LiDAR features at multiple scales in a monocular setup to predict dense scene flow. Its performance is much better in the critical regions where image-only and LiDAR-only methods are inaccurate. We verify our DeepLiDARFlow using the established data sets KITTI and FlyingThings3D and we show strong robustness compared to several state-of-the-art methods which used other input modalities. The code of our paper is available at https://github.com/dfki-av/DeepLiDARFlow.

==> alternate_abstract.tex <==
\begin{abstract}
In this paper we present DeepLiDARFlow, a novel deep learning architecture which fuses RGB and sparse LiDAR features in a monocular setup at multiple scales to predict scene flow. Scene flow is the 3D reconstruction of motion and geometry of a scene. Most available methods, variational as well as deep learning, use a pair of stereo images as input for full scene reconstruction. These methods depend a lot on the quality of images. RGB images can have regions with textureless objects, shadows, ill-conditioned light environment. LiDAR measurements are much less sensitive to such conditions. Fusion of LiDAR and RGB features can yield robust features which can improve the matching process and hence, yield better scene flow estimates. In the experiments section, we show even though DeepLiDARFlow uses a monocular image and sparse LiDAR as input, it still performs equivalent to LiDAR-Flow which uses a heavy hardware setup of stereo camera and LiDAR sensors. DeepLIDARFlow also outperforms various other state-of-the-art methods. Its performance is much better especially in the critical regions where image-only and LiDAR-only methods are inaccurate on KITTI 2015 and FlyingThings3D dataset.
\end{abstract}
